Learning the smoothness of noisy curves with application to online curve estimation

Combining information both within and across trajectories, we propose a simple estimator for the local regularity of the trajectories of a stochastic process. Independent trajectories are measured with errors at randomly sampled time points. Non-asymptotic bounds for the concentration of the estimator are derived. Given the estimate of the local regularity, we build a nearly optimal local polynomial smoother from the curves from a new, possibly very large sample of noisy trajectories. We derive non-asymptotic pointwise risk bounds uniformly over the new set of curves. Our estimates perform well in simulations. Real data sets illustrate the effectiveness of the new approaches.

==> head_val.tex <==
%% Packages
\RequirePackage[utf8]{inputenc}
\RequirePackage[T1]{fontenc}
\RequirePackage{amsthm,amsmath,amsfonts,amssymb, mathtools}
\mathtoolsset{showonlyrefs}
\RequirePackage[numbers]{natbib}
%\RequirePackage[authoryear]{natbib} %% uncomment this for author-year bibliography
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\RequirePackage{xcolor, graphicx}% uncomment this for including figures

\RequirePackage{enumerate}
\RequirePackage{comment}
\RequirePackage{ifthen}
\RequirePackage{subcaption}
\RequirePackage{siunitx}
\RequirePackage[ruled,vlined]{algorithm2e}

\usepackage{url}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% Uncomment next line to change            %%
%% the type of equation numbering           %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\numberwithin{equation}{section}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% For Axiom, Claim, Corollary, Hypothezis, %%
%% Lemma, Theorem, Proposition              %%
%% use \theoremstyle{plain}                 %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{stp}[section]

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{lemmaSM}{Lemma SM}

\DeclareSIUnit{\octet}{o}
\sisetup{binary-units,per-mode=symbol}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% For Assumption, Definition, Example,     %%
%% Notation, Property, Remark, Fact         %%
%% use \theoremstyle{remark}                %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\newtheorem{step}[stp]{Step}
%\newtheorem{???}{???}[???]
%\newtheorem{???}[???]{???}
%% Assumption
\newcounter{assumptionHt}
\newcounter{assumptionH}
\newcounter{assumptionE}
\newcounter{assumptionLP}
%
\newenvironment{assumptionHt}%
{%
\begin{enumerate}[({G}1)]%
    \setcounter{enumi}{\value{assumptionHt}}%
    }{%
    \setcounter{assumptionHt}{\value{enumi}}%
\end{enumerate}
}
%%
%%
\newenvironment{assumptionH}%
{%
\begin{enumerate}[({H}1)]%
    \setcounter{enumi}{\value{assumptionH}}%
    }{%
    \setcounter{assumptionH}{\value{enumi}}%
\end{enumerate}
}
%%
%%
\newenvironment{assumptionE}%
{%
\begin{enumerate}[({E}1)]%
    \setcounter{enumi}{\value{assumptionE}}%
    }{%
    \setcounter{assumptionE}{\value{enumi}}%
\end{enumerate}
}
%%
%%
\newenvironment{assumptionLP}%
{%
\begin{enumerate}[({LP}1)]%
    \setcounter{enumi}{\value{assumptionLP}}%
    }{%
    \setcounter{assumptionLP}{\value{enumi}}%
\end{enumerate}
}
%%
%%
\newcommand{\assrefHt}[1]{(\hyperref[#1]{G\ref{#1}})}
\newcommand{\assrefH}[1]{(\hyperref[#1]{H\ref{#1}})}
\newcommand{\assrefE}[1]{(\hyperref[#1]{E\ref{#1}})}
\newcommand{\assrefLP}[1]{(\hyperref[#1]{LP\ref{#1}})}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Please put your definitions here:        %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Probability
\newcommand{\asympp}{\approx}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\EEE}{\mathcal{E}}
\newcommand{\ET}{{\widetilde\EE}}
\newcommand{\PT}{{\widetilde\PP}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\PPP}{\mathcal{P}}
\newcommand{\EEB}{\mathbb{E}_{\mathcal B}}
\newcommand{\EEAn}{\mathbb{E}_{\mathcal A_n}}
\DeclareMathOperator{\Var}{Var}
\newcommand{\1}{\mathbf{1}}
%% Set
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\LL}{\mathbb{L}}
%% Different samples
\newcommand{\n}[1]{{n_{#1}}}
\newcommand{\N}[1]{{N_#1}}
% Regularity parameters
\newcommand{\degree}{\mathbf{d}}
\newcommand{\hdegree}{\hat {\mathbf{d}}}
\newcommand{\T}{{t_0}}
\newcommand{\HT}{H_\T}
\newcommand{\KT}{\degree}
\newcommand{\ST}{\varsigma_\T}
\newcommand{\hHT}{\widehat{H}_\T}
\newcommand{\hKT}{\hdegree}
\newcommand{\hST}{\widehat{\varsigma}_\T}
% Process
\newcommand{\Xtemp}[1]{%
	\ifthenelse{\equal{#1}{0}}
		{X^{(\n0)}}
		{
			\ifthenelse{\equal{#1}{1}}
				{X^{[\n1]}}
				{X^{(#1)}}
		}
	}
\newcommand{\hXtemp}[1]{%
	\ifthenelse{\equal{#1}{0}}
		{\widehat X^{(\n0)}}
		{
			\ifthenelse{\equal{#1}{1}}
				{\widehat X^{[\n1]}}
				{\widehat X^{(#1)}}
		}
	}
%
\newcommand{\Xp}[1]{X^{(#1)}}
\newcommand{\Xc}[1]{X^{[#1]}}
%
\newcommand{\X}[1]{{\Xtemp{#1}}}
\newcommand{\Xt}[1]{{\Xtemp{#1}_t}}
\newcommand{\XT}[1]{{\Xtemp{#1}_\T}}
\newcommand{\Xn}{{\Xtemp{n}}}
\newcommand{\Xtn}{{\Xtemp{n}_t}}
\newcommand{\XTn}{{\Xtemp{n}_\T}}       
%
\newcommand{\hX}[1]{{\hXtemp{#1}}}
\newcommand{\hXt}[1]{{\hXtemp{#1}_t}}
\newcommand{\hXT}[1]{{\hXtemp{#1}_\T}}
\newcommand{\hXn}{{\hXtemp{n}}}
\newcommand{\hXtn}{{\hXtemp{n}_t}}
\newcommand{\hXTn}{{\hXtemp{n}_\T}}       
%
\newcommand{\Ynm}{{Y^{(n)}_m}}
\newcommand{\Tnm}{{T^{(n)}_m}}
\newcommand{\Tnlm}{{T^{[n_1]}_m}}
\newcommand{\enm}{{\varepsilon^{(n)}_m}}
\newcommand{\unm}{{u^{(n)}_m}}

\newcommand{\Ostar}{\mathcal{O}}
\newcommand{\rhostar}{{\rho_*}}
\newcommand{\deltastar}{{\Delta_*}}
\newcommand{\epsilonstar}{\epsilon_*}



